From Monolithic Systems to Microservices: An Assessment Framework

Context. Re-architecting monolithic systems with Microservices-based architecture is a common trend. Various companies are migrating to Microservices for different reasons. However, making such an important decision like re-architecting an entire system must be based on real facts and not only on gut feelings. Objective. The goal of this work is to propose an evidence-based decision support framework for companies that need to migrate to Microservices, based on the analysis of a set of characteristics and metrics they should collect before re-architecting their monolithic system. Method. We designed this study with a mixed-methods approach combining a Systematic Mapping Study with a survey done in the form of interviews with professionals to derive the assessment framework based on Grounded Theory. Results. We identified a set consisting of information and metrics that companies can use to decide whether to migrate to Microservices or not. The proposed assessment framework, based on the aforementioned metrics, could be useful for companies if they need to migrate to Microservices and do not want to run the risk of failing to consider some important information.

==> figures/product-related-metrics.tex <==
\begin{table*}[h]
\caption{Product related metrics}
\label{tab:ProductBenefits}
\centering
\begin{tabular}
{@{}p{3.2cm}|p{14.2cm}@{}}
\hline 
\textbf{Characteristic} & \textbf{Metric }\\ \hline 
\multirow{12}{*}{Scalability/Performance} 
& \textbf{Response time:} The time between sending a request and receiving the corresponding response. It is a common metric to measure the performance impact of  approaches (\cite{SP1}\cite{SP4}, \cite{SP5}, \cite{SP6}, \cite{SP8}, \cite{SP9}, \cite{SP11}).\\
& \textbf{CPU utilization:} The percentage of time the CPU is not idle. Used to measure the performance. \cite{SP9} reports the relationship between number of VMs and the overall VMs utilization. In addition, \cite{SP11} analyzes the impact of the decision between VMs and containers on CPU utilization. \\
& \textbf{Path length:} The number of CPU instructions to process a client request. \cite{SP2} reports that the code-path length of a microservice application developed using Java with a hardware configuration of one Core, using as a bare process, docker host, and docker bridge are nearly two times higher than in the monolithic system. \\
& \textbf{Waiting time:} The time a service request spends in a waiting queue before it get processed. \cite{SP6}, \cite{SP10} discuss the relationship between waiting time and number of services. Furthermore, \cite{SP8} mentions an architecture design that half the waiting time compared to other design scenarios.\\
& \textbf{Impact of programming language:} Communication between microservices are network based. Most of the time is spend on network input and output operations rather than  processing of the request. Programming languages can influence the performances of the communication, due to the different ways that they implement the communication protocols. \cite{SP7} reports that, the programing language impact on the performance is negligible \cite{SP8}. \\
& \textbf{Usage of containers:} The usage of containers can influence the performance, since they need additional computational time compared to monolithic applications deployed in a single container. \cite{SP7} reports that the impact of containers on performance may not always be negligible. \\
& \textbf{Number of features per microservice:} \cite{SP10} points out that the number of features per microservice affect the scalability, influences the communication overhead and impacts the performance.\\
& \textbf{Number of requests per minute or second:} (also referred as throughput \cite{SP2,SP5,SP11} or average latency \cite{SP4,SP7}), is a performance metric. \cite{SP11} found that in their experimental setting, the container-based scenario could perform more request per second than the VM-based scenario. \\ 
\hline 
\multirow{3}{*}{Availability} 
& \textbf{Downtime:} \cite{SP4} highlights the long downtimes in microservices that took from several hours till 48 hours.  \\
& \textbf{Mean time to recover:} The mean time it takes to repair a failure and return back to operations. \cite{SP9} uses this metric to quantify availability.  \\
& \textbf{Mean time to failure:} The mean time till the first failure. \cite{SP9} uses this measure together with mean time to recover as a proxy for availability.  \\
\hline 
\multirow{3}{*}{Maintenance} 
& \textbf{Testability:} \cite{SP12} concludes that the loose coupling of microservices at the application's front-end level improves the testability.  \\
& \textbf{Complexity:} \cite{SP1}, \cite{SP5} notes that microservices reduce the complexity of a monolithic application by breaking it into a set of services. However, some development activities like testing may become more complex \cite{SP5}. Furthermore, \cite{SP7} state that the usage of different languages for different microservices increase the overall complexity. \\
\hline 
\multicolumn{2}{c}{} \\
\multicolumn{2}{c}{} 
\end{tabular}
\end{table*} 

==> sections/TheApproach.tex <==
\section{The Approach}
\label{Approach}

In this section, we will describe the two-step mixed-methods approach applied in this work. The approach is shown in Figure~\ref{fig:Approach}. 

The goal of this work is to understand which metrics are considered important by practitioners before and after the migration to Microservices. Therefore, we decided to conduct a survey based on semi-structured interviews. 

In order to avoid bias due to open-answer questions, we first performed a Systematic Mapping Study to identify a list of 
characteristics and measures considered in previous works for the identification of potential benefits and issues of the migration to Microservices. 




Then we conducted the survey among professionals to identify in practice which metrics they considered important before and after the migration, asking them to first report the metrics they considered useful as open questions, and then asking whether they considered the metrics used in the previous studies useful. 

In the next section (Section~\ref{MappingStudy}), we will report on the mapping study process, and in Section~\ref{Survey}, we will describe the survey design and the results obtained. 


\begin{figure}[H]
\centering 
\includegraphics[trim= 0 50 0 100, clip, width=\linewidth]{./figures/TheApproach.pdf}
\caption{The Approach}
\label{fig:Approach}
\end{figure}




==> sections/TheMappingStudy.tex <==
\section{Characteristics and measures investigated in empirical studies on Microservices}
\label{MappingStudy}

In this section, we aim to identify the characteristics and measures that companies should collect before re-architecting their monolithic system into Microservices in order to enablethem to make a rational decision based on evidence instead of gut feeling. Therefore, the goal of this work is two-fold: First, we aim to characterize which characteristics have been adopted in empirical studies to evaluate the migration from monolithic systems to Microservices. Second, we aim to map the measures adopted to measure the aforementioned characteristics. 

The contribution of this section can be summarized as follows: We identify and classify the different characteristics and measures that have been studied in empirical studies comparing monolithic systems with Microservices architectures. 
These measures will be used in the survey presented in Section~\ref{Survey}.

\subsection{Methodology}
\label{Methodolody}
Here, we will describe the protocol followed in this Systematic Mapping Study. We will define the goal and the research questions (Section~\ref{RQs}) and report the search strategy approach (Section~\ref{SearchStrategy}) based on the guidelines defined by Petersen et al.~\cite{Petersen2008,Petersen2015} and the ``snowballing'' procedure defined by Wohlin~\cite{Wohlin2014}. We will also outline the data extraction and the analysis (Section~\ref{DataExtraction}) of the corresponding data. The adopted protocol is depicted in Figure~\ref{fig:SSProcess}.%\ref{fig:SMProcess}. 

%\begin{figure*}[h]
%\centering
%\includegraphics[trim= 0 250 0 100,  clip, width=0.7\linewidth]{./figures/SMProcess.pdf}
%\caption{The Systematic Mapping process}
%\label{fig:SMProcess}
%\end{figure*}
 
\subsubsection{Goal and Research Questions}
\label{RQs}
The goal of this Systematic Mapping Study is to analyze the characteristics and measures considered in empirical studies that evaluated the migration from monolithic systems to Microservices or that evaluated Microservices.
For this purpose, we addressed the following research questions (RQs): \\
\textbf{RQ1. }Which characteristics have been investigated during the analysis of the migration from monolithic systems to Microservices architectures? \\
With this RQ, we aim to classify the characteristics reported by the empirical studies that analyzed the migration from monolithic systems to Microservices. \\ \\
\textbf{RQ2. }What measures have been adopted to empirically evaluate the characteristics identified in RQ1? \\
For each characteristic, we identified the measures adopted for the evaluation of the migration to Microservices. \\ \\
\textbf{RQ3. }What effects have been measured after the migration to Microservices? \\
With this RQ, we aim to analyze the results reported in the measures identified in RQ2. For example, we aim to understand whether the selected studies agree about the decreased maintenance effort of Microservices expected by numerous practitioners~\cite{TaibiIEEECloud}. 


\subsubsection{Search Strategy}
\label{SearchStrategy}
We adopted the protocol defined by Petersen et al.~\cite{Petersen2008, Petersen2015} for a Systematic Mapping Study and integrated it with the systematic inclusion of references --- a method also referred to as ``snowballing''--- defined by Wohlin~\cite{Wohlin2014}.

The protocol involves the outline of the search strategy including bibliographic source selection, identification of inclusion and exclusion criteria, definition of keywords, and the selection process that is relevant for the inclusion decision. The search and selection process is depicted in Figure~\ref{fig:SSProcess}. 

\begin{figure}[H]
\centering
\includegraphics[trim= 250 20 150 0, clip, width=0.55\linewidth]{./figures/SearchSelectionProcess.pdf}
\caption{The search and selection process}
\label{fig:SSProcess}
\end{figure}

\textbf{Bibliographic Sources}. We selected the list of relevant bibliographic sources following the suggestions of Kitchenham and Charters~\cite{Kitchenham2007}, since these sources are recognized as the most representative in the software engineering domain and are used in many reviews. The list includes: \textit{ACM Digital Library, IEEEXplore Digital Library, Science Direct, Scopus, Google Scholar, Citeseer Library, Inspec, Springer Link}.

\textbf{Inclusion and Exclusion Criteria}. We defined inclusion and exclusion criteria based on the papers' title and abstract in order to identify the most relevant papers. We obtained the final criteria by means of refinements from an initial set of inclusion and exclusion criteria. 

\textit{Inclusion criteria}. The selected papers fulfilled \textbf{all} of the following criteria: 
\begin{itemize}
\itemsep0em 
%\item The study must have been published either in a peer-reviewed journal or in conference proceedings before the end of July 2017\footnote{It is possible that some indexes were not up to date when we carried out the search.}.
%\item If the study is published in more than one journal or conference, only the most recent version of the study has to considered.
\item Relation to Microservices migration can be deduced.
\item Study has to provide empirical evidence (measures) between the previous monolithic system and the refactored Microservices-based system. Examples of measures may include maintenance effort, costs, infrastructure costs, response time, and others. 
\end{itemize} 

\textit{Exclusion criteria}. Selected papers not fulfilling \textbf{any} of the following criteria were left out: 
\begin{itemize}
\itemsep0em 
\item Not written in English.
\item Duplicated paper (only the most recent version was considered).
%\item Not peer-reviewed (such as books or book chapters, presentations, call for papers, keynote speeches, prefaces, gray literature, etc.);
\item Not published in a peer-reviewed journal or conference proceedings before the end of July 2017\footnote{It is possible that some indexes were not up to date when we carried out the search.}.
\item Short paper, workshop paper, and work plan (i.e., paper that does not report results).
%\item Not related to cloud native migration.
\end{itemize}

\textbf{Definition of Search Keywords}. We defined search keywords based on the PICO~\cite{Kitchenham2007} structure\footnote{The PICO structure includes as terms: Problem/Patient/Population, Intervention/Indicator, Comparison, Outcome} as reported in Table~\ref{tab:SearchKeywords}. 

\begin{table}[H]
\centering
\caption{Definition of Search Keywords} 
\label{tab:SearchKeywords} 
\footnotesize
\begin{tabular}[ht]
{@{}p{2.7cm}|p{7cm}@{}}
\hline
\textbf{Population} & Microservice; micro-service; ``micro service'' \\ \hline
\textbf{Intervention} & migration; evaluation; adoption \\ \hline
\textbf{Comparison} & monolith \\ \hline
\textbf{Outcome} & framework; impact; factor; driver \\ \hline
\end{tabular}
\end{table}

Based on these terms, we formulated the following search string: \\
(microservi* OR micro-servi* OR ``micro servi*'') \\
\textbf{AND} 
(migration OR evaluation OR adoption OR compar*) \\
\textbf{AND} (monolith*) \\
\textbf{AND} (framework OR impact OR factor* OR driver* Or analy* OR metric* OR measure*). 

The symbol * allowed us to capture possible variations in the search terms such as plurals and verb conjugations. 

\textbf{Search and Selection}. The application of the search keywords returned 142 unique papers. Next, we applied the inclusion and exclusion criteria to the retrieved papers. As suggested by Kitchenham and Brereton~\cite{Kitchenham2013}, we first tested the applicability of the inclusion and exclusion criteria:
\begin{enumerate}
\item A set of 15 papers was selected randomly from the 142 papers. 
\item Three authors applied the inclusion and exclusion criteria to these 15 papers, with every paper being evaluated by two authors.
\item On three of the 15 selected papers, two authors disagreed and a third author joined the discussion to clear up the disagreements.
\end{enumerate}
The refined inclusion and exclusion criteria were applied to the remaining 127 papers. Out of 142 initial papers, we excluded 70 by title and abstract and another 61 after a full reading process. We settled on 11 papers as potentially relevant contributions.
In order to retrieve all relevant papers, we additionally integrated the procedure of also taking into account forward and backward systematic snowballing~\cite{Wohlin2014} on the 11 remaining papers. As for backward snowballing, we considered all the references in the papers retrieved, while for the forward snowballing we evaluated all the papers referencing the retrieved ones, which resulted in one additional relevant paper. Table~\ref{tab:SelectionResults} summarizes the search and selection results obtained. 

This process resulted in us retaining 12 papers for the review. The list of these 12 papers is reported in Table~\ref{tab:SelectedPaper}.

\begin{table}[ht]
\centering
%\captionsetup[table]{skip=5pt}
\caption{Search and Selection Results} 
\label{tab:SelectionResults} 
\footnotesize
\begin{tabular}
{@{}p{6cm}|p{2cm}@{}}
\hline
\textbf{Step} & \textbf{\# papers} \\ \hline
Retrieval from bibliographic sources & 142 \\ \hline
Inclusion and exclusion criteria & -70\\ \hline
Full reading & -61 \\ \hline
Snowballing & 1 \\ \hline
\textbf{Papers identified} & \textbf{12} \\ \hline
\end{tabular}
\end{table}
\subsubsection{Data Extraction}
\label{DataExtraction}
Data addressing our RQs was extracted from each of the 12 papers that were ultimately included in the review. For this purpose, two of the authors extracted the data independently and then compared the results. If the results differed, a third author verified the correctness of the extraction. 

Our goal was to collect data that would allow us to characterize the measures that can be used to evaluate the migration to Microservices. Two groups of data were extracted from each primary study: 
\begin{itemize}
\itemsep0em 
\item \textit{Context data}. Data showing the context of each selected study in terms of: the goal of the study, the source of the data studied, the number of Microservices developed, the application area (i.e., insurance system, banking system, room reservation, ...), and the programming language of the studied system(s).
\item \textit{Empirically Evaluated Characteristics}. Data related to the characteristics under study (e.g., maintenance, cost, performance, ...) and the measures adopted in the studies (e.g., number of requests per minute, cyclomatic complexity, ...). 
\end{itemize}

\subsection{Data Synthesis}
\label{Synthesis}
The data extracted from each paper was aggregated and summarized by two of the authors in order to better answer our RQs. First, we identified and classified the set of characteristics to answer RQ2. Before identifying the technique to be used in the classification, we first screened the characteristics mentioned in the papers. Since the papers clearly reported the characteristics under study, using the same terminology (e.g., performance was always referred to as performance, maintenance as maintenance, and so on), we simply took all the categories as they were. 

As for the measures adopted for measuring each characteristic, we followed the same process. In this case, the papers adopted different terms for similar measures, or in some cases only different units of measurement (e.g., number of requests per minute instead of number of requests per hour). 
In order to classify similar measures, three authors proposed their own classification independently. Then they discussed the final classification in a workshop so as to resolve any incongruences. 

\subsubsection{Study Replicability}
\label{Replicability}
In order to allow replication and extension of our work, we prepared a replication package\footnote{The raw data is temporarily stored on Google Drive: https://drive.google.com/open?id=1GNnDMmNckRgrxk6yEw8wsiHOT2iFDWEj. The data will be moved to a permanent repository in case of acceptance.} for this Systematic Mapping Study, including the complete results obtained. 

\begin{table*}[!h]
\caption{Selected Papers}
\label{tab:SelectedPaper}
\centering
\footnotesize
\begin{tabular}
{@{}p{1cm}|p{7cm}|p{2.5cm}|p{0.8cm}@{}}
\hline 
\textbf{Study ID} & \textbf{Title} & \textbf{Author} & \textbf{Year} \\ \hline 
\cite{SP1}	&	Evaluating the monolithic and the Microservice architecture pattern to deploy web applications in the cloud	&	Villamizar M. et al. &	2015	\\ \hline 
\cite{SP2}	&	Workload characterization for Microservices	&	Ueda T. et al.		&	2016
\\ \hline 
\cite{SP3}	&	Infrastructure Cost Comparison of Running Web Applications in the Cloud Using AWS Lambda and Monolithic and Microservice Architectures	&	Villamizar M. et al. &	2016
\\ \hline 
\cite{SP4}	&	Gremlin: Systematic Resilience Testing of Microservices	&	Heorhiadi V. et al.	&	2016	\\ \hline 
\cite{SP5}	&	An Architecture to Automate Performance Tests on Microservices	&	De Camargo A. et al.		&	2016	\\ \hline 
\cite{SP6}	&	Efficiency analysis of provisioning Microservices	&	Khazaei H. et al.		&	2016	\\ \hline 
\cite{SP7}	&	Investigation of impacts on network performance in the advance of a Microservice design	&	Kratzke N. and Quint P.C.	&	2017	\\ \hline 
\cite{SP8}	&	A scalable routing mechanism for stateful Microservices	&	Do N.H. et al.		&	2017	\\ \hline 
\cite{SP9}	&	Performance evaluation of massively distributed Microservices based applications	&	Gribaudo M. et al.		&	2017	\\ \hline 
\cite{SP10}	&	Workload-Based Clustering of Coherent Feature Sets in Microservice Architectures	&	Klock S. et al.		&	2017	\\ \hline 
\cite{SP11}	&	Performance comparison between container-based and VM-based services	&	Salah T. et al.	&	2017 \\ \hline 	
\cite{SP12}	&	Guidelines for adopting frontend architectures and patterns in Microservices-based systems	&	Harms H. et al.	&	2017 \\ 
\hline
\end{tabular}
\end{table*}

\subsection{Results}
\label{sec:mappResults}
In this section, we will answer our research questions based on the data extracted from each selected paper.

In order to get a general overview of the selected papers, we extracted information on publication year, type, and venue for each publication. 
We are aware that the limited number of selected studies is not enough to draw statistical conclusions. However, the results of this RQ help to understand the growing trend of works in this domain. 

\textbf{Publication per year}. The term ``Microservice'' was introduced in 2012. Therefore, we did not consider any work before 2012. The scientific interest in Microservices and in particular in empirical studies evaluating the migration from monolithic systems has increased in recent years. The twelve selected papers were all published between 2015 and 2017.
% , as shown in Figure~\ref{fig:YearDistribution}. 
No relevant papers were found before 2015.

\textbf{Publication type and venue}. The selected papers appeared in eleven different publication venues, including ten international conferences and one national conference. Specifically, the papers were published in: Symposium on the Foundations of Software Engineering (FSE 2015), International Symposium on Workload Characterization (IISWC 2016), International Symposium on Cluster, Cloud, and Grid Computing (CCGrid 2016), International Conference on Distributed Computing Systems (ICDCS 2016), International Conference on Information Integration and Web-based Applications and Services (iiWAS 2016), International Conference on Cloud Computing Technology and Science (CloudCom 2016), International Conference on Cloud Computing and Services Science (CLOSER 2016), Conference on Innovations in Clouds, Internet and Networks (ICIN 2017), European Conference on Modelling and Simulation (ECMS 2017), International Conference on Software Architecture (ICSA 2017), Conference on Innovations in Clouds, Internet and Networks (ICIN 2017) and Colombian Computing Conference (10CCC 2015). 

% \begin{figure}[h]
% \centering
% %\includegraphics[width=\linewidth]{./figures/PublicationYear.pdf}

% \begin{tikzpicture}
% \begin{axis}[
% 	height=1.6in,
%     width=0.9\linewidth,
%     xtick={2015,2016,2017},
%     xticklabels={2015,2016,2017},
%     ytick={1,2,3,4,5,6},
%     label style={font=\footnotesize},
%     every axis/.append style={font=\footnotesize},
% 	xlabel=Year,
%     ylabel=Number of Papers,
%     bar width=20,
% 	ybar %interval=0.5,
% ]
% \addplot coordinates {(2015,1) (2016,5) (2017,6)};
% %\legend{papers}
% \end{axis}
% \end{tikzpicture}
% \caption{Paper distribution per year}
% \todo[inline]{This figure is very sparse, so it could be contra-productive-I suggest to remove it} @Davide. I Agree :-)
% \label{fig:YearDistribution}
% \end{figure}

\subsubsection{Studied Characteristics (RQ1)}
\label{RQ2}
In order to better answer RQ1, we briefly present an overview of the papers in terms of the research strategy, the adopted evaluation approach, and the main purpose of each study. 

\textbf{Research strategy}. Comparing the different research strategies, evaluation research (\cite{SP1}, \cite{SP2}, \cite{SP3}, \cite{SP11}, \cite{SP12}) and solution proposal (\cite{SP4}, \cite{SP5}, \cite{SP8}, \cite{SP9}, \cite{SP10}) are the most common strategies (five papers each), while the remaining papers conducted validation research (\cite{SP6}, \cite{SP7}). 
Nevertheless, all papers have in common that their empirical validation is based on case studies.

The selected studies focus mainly on analyzing the migration benefits and challenges (\cite{SP1}, \cite{SP3}, \cite{SP11}, \cite{SP12}). The other subjects on which they focus are distributed system architectures (\cite{SP2}, \cite{SP12}) and evaluation models and frameworks to validate the performance (\cite{SP4}, \cite{SP5}, \cite{SP6}, \cite{SP7}, \cite{SP9}, \cite{SP10}). 

\textbf{Addressed characteristics}. In order to better classify the results, we distinguish between product and process characteristics. Moreover, we also consider cost as an organizational characteristic.
The selected studies mainly focus on product characteristics (\cite{SP1}, \cite{SP2}, \cite{SP4}, \cite{SP5}, \cite{SP6}, \cite{SP7}, \cite{SP8}, \cite{SP9}, \cite{SP10}, \cite{SP11}, \cite{SP12}) or on process characteristics (\cite{SP1}, \cite{SP3}, \cite{SP9}, \cite{SP11}, \cite{SP12}).
However, five of them focus on both (\cite{SP1}, \cite{SP4}, \cite{SP9}, \cite{SP11}, \cite{SP12}). 
Only three papers (\cite{SP1}, \cite{SP3}, \cite{SP5}) investigated the issue of cost comparison. Only \cite{SP1} evaluated all the characteristics considered in this review. 

Regarding the product characteristics, we identified four sub-characteristics: performance, scalability, availability, and maintenance. We also divided cost comparison into personnel and infrastructure costs. 

The most frequently addressed characteristic is performance (see Table \ref{tab:ProcessBenefits}). In detail, the papers \cite{SP1}, \cite{SP2}, \cite{SP4}, \cite{SP5}, \cite{SP6}, \cite{SP7}, \cite{SP8}, \cite{SP9}, \cite{SP11} have a focus on performance. This is followed by scalability, which is discussed by the papers \cite{SP2},\cite{SP4},\cite{SP5},\cite{SP6},\cite{SP7},\cite{SP8}, \cite{SP10}, and \cite{SP11}.
Other characteristics like availability (\cite{SP4}, \cite{SP9}) or maintenance (\cite{SP1},\cite{SP5}, \cite{SP7}, \cite{SP12}) are considered only in a few papers. 

Overall, we identified the following characteristics as reported in Tables \ref{tab:ProductBenefits}, \ref{tab:ProcessBenefits}, and \ref{tab:CostComparison}:
\begin{itemize}
\item \textbf{Product}
\begin{itemize}
\item Performance
\item Scalability
\item Availability
\item Maintenance
\end{itemize}
\item \textbf{Process}
\item \textbf{Cost}
\begin{itemize}
\item Personnel Cost
\item Infrastructure Cost
\end{itemize}
\end{itemize}

\subsubsection{Measures Adopted to Evaluate Characteristics (RQ2)
%Which metrics have been adopted to evaluate the characteristics identified in RQ2 (RQ3)
}
\label{RQ3}
Two authors analyzed each paper and identified 18 measures for the three main characteristics considered in RQ1, as depicted in Figure~\ref{fig:RQ2} and reported in Tables~\ref{tab:ProductBenefits}, \ref{tab:ProcessBenefits}, and~\ref{tab:CostComparison}. 

\textbf{Product-related measures}. 
We identified 13 measures (Table~\ref{tab:ProductBenefits}) for the four identified sub-characteristics (performance, scalability, availability, and maintenance).

From the obtained results, we can see that the highest number of measures is related to performance and scalability, where we identified a total of nine studies referring to them. Among them, response time, number of requests per minute or second, and waiting time are the most commonly addressed measures. 
For availability, we derived only three measures and for maintainability only two. 

\textbf{Process-related measures}. Seven studies investigated the migration process using three factors: development independence between teams, usage of continuous delivery, and reusability (Table~\ref{tab:ProcessBenefits}). These three factors can be considered as ''Boolean measures'' and can be used by companies to understand whether their process can be easily adapted to the development of Microservices-based systems. 

Existing independent teams could easily migrate and benefit from the independence freedom provided by Microservices. Continuous delivery is a must in Microservices-based systems. The lack of a continuous delivery pipeline eliminates most of the benefits of Microservices.
Reusability is amplified in Microservices. Therefore, systems that need to reuse the same business processes can benefit more from Microservices, while monolithic systems in which there is no need to reuse the same processes will not experience the same benefits. 

Besides the analyzed characteristics, the papers also discuss several process-related benefits of the migration. Technological heterogeneity, scalability, continuous delivery support, and simplified maintenance are the most frequently mentioned benefits. Furthermore, the need for recruiting highly skilled developers and software architects is considered as a main motivation for migrating to Microservices. 

\textbf{Cost-comparison-related measures}. 
As for this characteristic, three studies include it in their analysis and consider three measures for the comparison (Table~\ref{tab:CostComparison}). 

\begin{table}[H]
\caption{Product-related measures}
\label{tab:ProductBenefits}
\centering
\scriptsize
\begin{tabular}
{@{}p{2cm}|p{1cm}|p{8.5cm}@{}}
\hline 
\textbf{Characteristic} & \textbf{Papers} & \textbf{Measures}\\ \hline 
\multirow{5}{*}{\pbox{2.2cm}{Performance}} 
& 58\% & \textbf{Response time:} The time between sending a request and receiving the corresponding response. This is a common metric for measuring the performance impact of approaches (\cite{SP1}\cite{SP4}, \cite{SP5}, \cite{SP6}, \cite{SP8}, \cite{SP9}, \cite{SP11}).\\
& 16\% & \textbf{CPU utilization:} The percentage of time the CPU is not idle. Used to measure performance. \cite{SP9} reports the relationship between the number of VMs and the overall VMs utilization. In addition, \cite{SP11} analyzes the impact of the decision between VMs and containers on CPU utilization. \\
& 16\% & \textbf{Impact of programming language:} Communication between Microservices is network-based. Most of the time is spent on network input and output operations rather than on processing of the request. Programming languages can influence communication performance due to the different ways that they implement the communication protocols. \cite{SP7} reports that the impact of the programming language on performance is negligible \cite{SP8}. \\
& 8\% & \textbf{Path length:} The number of CPU instructions to process a client request. \cite{SP2} reports that the length of the code path of a Microservice application developed using Java with a hardware configuration of one core, using a bare process, docker host, and docker bridge, is nearly twice as high as in a monolithic system. \\
& 8\% & \textbf{Usage of containers:} The usage of containers can influence performance, since they need additional computational time compared to monolithic applications deployed in a single container. \cite{SP7} reports that the impact of containers on performance might not always be negligible. \\
\hline 
\multirow{3}{*}{\pbox{2.2cm}{Scalability}} 
& 41\% & \textbf{Number of requests per minute or second:} (also referred to as throughput \cite{SP2,SP5,SP11} or average latency \cite{SP4,SP7}), is a performance metric. \cite{SP11} found that in their experimental setting, the container-based scenario could perform more requests per second than the VM-based scenario. \\ 
& 25\% & \textbf{Waiting time:} The time a service request spends in a waiting queue before it gets processed. \cite{SP6}, \cite{SP10} discuss the relationship between waiting time and number of services. Furthermore, \cite{SP8} mentions an architecture design that halves the waiting time compared to other design scenarios.\\
& 8\% & \textbf{Number of features per Microservice:} \cite{SP10} points out that the number of features per Microservice affects scalability, influences communication overhead, and impacts performance.\\
\hline 
\multirow{3}{*}{Availability} 
& 8\% & \textbf{Downtime:} \cite{SP4} highlights long downtimes in Microservices, which lasted from several hours to 48 hours. \\
& 8\% & \textbf{Mean time to recover:} The mean time it takes to repair a failure and return back to operations. \cite{SP9} uses this measure to quantify availability. \\
& 8\% & \textbf{Mean time to failure:} The mean time until the first failure. \cite{SP9} uses this measure together with mean time to recover as a proxy for availability. \\
\hline 
\multirow{3}{*}{Maintenance} 
& 25\% & \textbf{Complexity:} \cite{SP1}, \cite{SP5} notes that Microservices reduce the complexity of a monolithic application by breaking it down into a set of services. However, some development activities like testing may become more complex \cite{SP5}. Furthermore, \cite{SP7} state that the usage of different languages for different Microservices increases the overall complexity. \\
& 8\% & \textbf{Testability:} \cite{SP12} concludes that the loose coupling of Microservices at the application's front-end level improves testability. \\ \hline 
\end{tabular}
\end{table} 


\begin{table}[H]
\caption{Process-related factors}
\label{tab:ProcessBenefits}
\centering
\scriptsize
\begin{tabular}
{@{}p{2cm}|p{1cm}|p{8.5cm}@{}}
\hline 
\textbf{Characteristic} & \textbf{Papers} & \textbf{Measures }\\ \hline 
\multirow {3}{*}{\pbox{2.2cm}{Process-related\\benefits}} 
& 41\% & \textbf{Development independence between teams:} The migration from a monolithic architecture to a Microservices- oriented one changes the way in which the development team is organized. Typically, a development team is reorganized around the Microservices into small, cross-functional, and self-managed teams \cite{SP1}, \cite{SP3}, \cite{SP4}, \cite{SP9}, \cite{SP12}. \\    

& 8\% & \textbf{Continuous delivery:} \cite{SP1} notes that the deployment in a Microservices environment is more complex, given the high number of deployment targets. Hence, the authors of \cite{SP1} suggest automating the deployment as much as possible. \\

& 8\% & \textbf{Reusability:} Microservices are designed to be independent of their environment and other services \cite{SP11}. This facilitates their reusability.\\
\hline 
\end{tabular}
\end{table} 

\begin{table}[H]
\caption{Cost-related measures}
\label{tab:CostComparison}
\centering
\scriptsize
\begin{tabular}
{@{}p{2cm}|p{1cm}|p{8.5cm}@{}}
\hline 
\textbf{Characteristic} & \textbf{Papers} & \textbf{Measure }\\ \hline 
\multirow {3}{*}{Personnel Cost} 
& 8\% & \textbf{Development costs:} \cite{SP5} argues that Microservices reduce the development costs given that complex monolithic applications are broken down into a set of services that only provide a single functionality. Furthermore, most changes affect only one service instead of the whole system. \\
\hline 
\multirow {3}{*}{\pbox{2.2cm}{Infrastructure\\Cost}} 
& 16\% & \textbf{Cost per hour:} Is a measure used to determine the infrastructure costs \cite{SP1}. According to the experiment done in \cite{SP3}, the Microservices architecture had lower infrastructure costs compared to monolithic designs. \\
& 8\% & \textbf{Cost per million requests:} In comparison to cost per hour, this measure is based on the number of requests / usage of the infrastructure. \cite{SP3} uses the infrastructure costs of a million requests to compare different deployment scenarios. \\
\hline
\end{tabular}
\end{table} 

\begin{figure*}[ht]
\centering
\includegraphics[trim= 20 0 0 -20, clip, width=1.05\linewidth]{./figures/RESULT-TREE.pdf}
\caption{Summary of Microservices characteristics and measures (RQ2 and RQ3)}
\label{fig:RQ2}
\end{figure*}


\subsubsection{Microservices Migration Effects (RQ3)}
The analysis of the characteristics and measures adopted in the empirical studies considered in this review allowed us to classify a set of measures that are sensitive to variations when migrating to Microservices. The detailed mapping between the benefits and issues of each measure is reported in Table~\ref{tab:ProductBenefits}. 

\textbf{Product Characteristics}. Regarding product characteristics, performance is slightly reduced in Microservices. 

When considering the different measures adopted to measure \textbf{performance}, the usage of containers turned out to decrease performance. This is also confirmed by the higher number of CPU instructions needed to process a client request (path length), which is at least double that of monolithic systems and therefore results in high CPU utilization. 
However, the impact of the usage of different programming languages in different services is negligible. Even if different protocols have different interpreters for different languages, the computational time is comparable. 

When considering \textbf{scalability}, Microservices-based systems outperform monolithic systems. Compared to monolithic systems, response time is lower in Microservices. However, when the number of requests grows, Microservices are easier to scale, mainly because of their relatively small size, and can keep on serving clients with the same response time, whereas monolithic systems commonly decrease their response time when the number of requests peaks. 

Taking into account \textbf{availability}, \cite{SP4} and \cite{SP9} report that Microservices can be affected by higher availability problems. This is due to the higher number of connected components, which, in the event of a failure, could disrupt the whole system. Although several practitioners claim the opposite - that Microservices are more robust, and that in the event of the failure of one Microservice, the remaining part of the system will still be available~\cite{Soldani2018}\cite{TaibiIEEECloud} - the systems analyzed by~\cite{SP4} and \cite{SP9} seemed to suffer from lower availability compared to the previous monolithic systems.

\textbf{Maintenance} is considered more expensive in the selected studies. The selected studies agree that the maintenance of a single Microservice is easier than maintaining the same feature in Microservices. However, testing is much more complex in Microservices ~\cite{SP7}, and the usage of different programming languages, the need for orchestration, and the overall system architecture increase the overall maintenance effort. 


\textbf{Cost-related measures}
The development of Microservices-based systems is reported to be more expensive than the development of monolithic systems~\cite{SP5}. Moreover, infrastructure costs are usually also higher for Microservices than for monolithic systems~\cite{SP1}\cite{SP3}. 










